Empirical Game-Theoretic Analysis: A Survey

In the empirical approach to game-theoretic analysis (EGTA), the model of the game comes not from declarative representation, but is derived by interrogation of a procedural description of the game environment. The motivation for developing this approach was to enable game-theoretic reasoning about strategic situations too complex for analytic specification and solution. Since its introduction over twenty years ago, EGTA has been applied to a wide range of multiagent domains, from auctions and markets to recreational games to cyber-security. We survey the extensive methodology developed for EGTA over the years, organized by the elemental subproblems comprising the EGTA process. We describe key EGTA concepts and techniques, and the questions at the frontier of EGTA research. Recent advances in machine learning have accelerated progress in EGTA, and promise to significantly expand our capacities for reasoning about complex game situations.

==> alpharank.tex <==


More recently, a related solution concept called \term{\alpharank} was proposed by \citet{omidshafiei2019alpha}. $\alpha$-Rank is a principled evolutionary dynamics methodology that is based on a new game theoretic solution concept, Markov-Conley Chains, that provides a ranking of agents or strategies under study. The approach is tractable and scales in the number of agents, goes beyond pairwise interactions and can handle both symmetric and asymmetric games.

The intuition behind the approach is as follows (for a detailed exposition see \citet{omidshafiei2019alpha}): in potential games, the potential function decreases under the standard dynamics such as best-responses, and guides players towards standard solution concepts of equilibria such as the Nash equilibrium. Unfortunately, this is not so for agents involved in the more general classes of games we are typically interested in evaluating. In the \term{\alpharank} method the goal is to identify the non-trivial and irreducible behaviors of a dynamical system, these are the behaviors that cannot be partitioned more finely in a way that respects the dynamics.  Specifically, just as John Nash used one of the most advanced topological results of his time, i.e., Kakutani's fixed point theorem, as the basis for the Nash solution concept, \term{\alpharank} employs Conley's Fundamental Theorem of Dynamical Systems as the basis of its solution concept. What Conley’s theorem says, informally, is that the space on which a dynamical system operates can be decomposed into two parts: a gradient-like part that is led to a recurrent part. In game-theoretic terms, Conley’s Theorem says that every game is a potential game, if only we change our solution concept from equilibria to recurrent sets.

Although \term{\alpharank} wishes to study these recurrent sets, it’s actually difficult to do so in practice because we don’t have an exact handle on their geometry or the behavior of the dynamics inside them. In practice, it’s hard even to make informed guesses about when the dynamics have converged to such a recurrent set.
To resolve this, \term{\alpharank} focuses onto a meaningful analog with similar limiting dynamics, but one which we can  tractably analyze. It uses a discrete-time discrete-space approximation, which is the \emph{response graph} of the game, whose nodes are the set of pure strategy profiles. This response graph has directed edges towards a deviating player’s new strategy, if it’s a better response against the other players, compared to her old strategy. We show an example in figure \ref{fig:exampleresponse} for a 2 player game with 3 strategies per player. The payoffs are shown on the left, and the response graph on the right.

\begin{figure}
    \centering
    \includegraphics[width=8cm]{figs/exampleresponse.png}
    \caption{The $\alpha$-Rank algorithm summarized.}
    \label{fig:exampleresponse}
\end{figure}

In essence, $\alpha$-Rank defines an irreducible Markov chain over the strategy set $S$, which results in the response graph. The ordered masses of this Markov chain's unique stationary distribution $\boldsymbol{\pi}$ yield the solution concept and provide strategy profile rankings. Figure \ref{fig:ARank} summarizes the involved steps.

Markov-Conley chain (MCCs) are Markov chains over the sink strongly connected components of the response graph. They are essentially an approximation of the recurrent components of our continuous-time dynamics, hence the connection to Conley's Theorem. In Figure \ref{fig:exampleresponse} we hace highlighted the two MCCs in blue. The MCC in the top-left consists of a cycle over four nodes, and the bottom right one is an isolated sink node
In essence, MCCs are used as a computational handle that aims to mimic the long-term behavior of dynamics in general games, in a tractable manner.

MCCs are attractive from a computational standpoint: they can be found efficiently in any game by computing the sink components of the response graph. This addresses one of the key criticisms of Nash equilibria. Unfortunately, similar to Nash, MCCs face an equilibrium selection problem, and as such we may have many MCCs, and the dynamics can converge to any of them. To resolve the MCC selection issue we introduce noise in the system.
We perturb the system such that a random walk on the response graph can actually climb upward on the potential hills, and effectively hop between MCCs with a very small probability.
What this means is that the overall Markov chain is irreducible, and so has a unique stationary distribution. This stationary distribution indicates the average time players spend in each MCC, and gives us our rankings.


The remarkable finding is that these perturbed dynamics correspond to a discrete-time evolutionary process. These evolutionary processes have been well-studied in the literature for pairwise symmetric games, but \term{\alpharank} extends them to the case of n-player asymmetric interactions, which are more general. The basic idea in these evolutionary dynamics is to model a selection-mutation process over a set of interacting populations.
Individuals sampled from each population play an n-player game, and the strongest individuals either reproduce, or, with a very small probability, mutate.


Specifically, the propagation of strong agents is driven by a selection function, which you can see on the bottom right of Figure \ref{fig:evoARank}, that compares the fitness of a resident agent \tau with a competing agent \sigma.
The intensity of selection, or the so-called ranking-intensity value $\alpha$, determines the probability that a mutant overtakes a population.
A low ranking-intensity, $\alpha$, corresponds to the case of weak selection. 
A large $\alpha$ ensures that only the strongest strategies survive. Under the large $\alpha$ limit, this evolutionary model converges exactly to the perturbed MCC model we outlined previously, and yields the ranking method which is called \term{\alpharank}.

\begin{figure}
    \centering
    \includegraphics[width=8cm]{figs/Arankevo.png}
    \caption{The $\alpha$-Rank algorithm summarized.}
    \label{fig:evoARank}
\end{figure}


%\kt{expand on these now.}


Based on the dynamical solution concept of MCCs and the evolutionary model, we can now detail the alpha-Rank method, illustrated in Figure \ref{fig:ARank}

\begin{figure}
    \centering
    \includegraphics[width=8cm]{figs/alpharankmethod.png}
    \caption{The $\alpha$-Rank algorithm summarized.}
    \label{fig:ARank}
\end{figure}

The first step is to construct the empirical game or payoff table. We can then define a Markov chain whose states correspond to the agents being evaluated in the empricial game.
Next we compute the transition matrix $C$ over this Markov chain according to our selection-mutation model.
Finally, since our Markov chain is irreducible, we can compute a unique stationary distribution $pi$ and rank our agents accordingly using the masses of this distribution.

For full formal details we refer to \cite{omidshafiei2019alpha}.

In Figure \ref{fig:ARankAlphaGo} we provide an example on AlphaGo. The empirical game here corresponds to a 2-player symmetric game with 7 AlphaGo variants, each agent using a different combination of rollouts, value networks, and policy networks.
The game payoffs correspond to the win ratios of the pairwise match-ups of these agents.
On the left we have our discrete-time Markov chain, where each node is a distinct agent, with the node color indicating the mass of the stationary distribution on that agent.
\term{\alpharank} is quite conclusive here, in the sense that the top agent, $AlphaGo(rvp)$, attains all of the stationary distribution mass, dominating the other agents.

\begin{figure}
    \centering
    \includegraphics[width=8cm]{figs/alphagoEGTA.png}
    \caption{The $\alpha$-Rank algorithm summarized.}
    \label{fig:ARankAlphaGo}
\end{figure}

%A final point here is that the Markov chain on the left summarizes the  dynamics of all agents, simultaneously on a single figure.
%Compare this to our earlier evolutionary game theory models, where one would have to individually analyze all possible 2-faces of the simplex, of which there are 35 total here.
%This makes for a substantial reduction in the amount of analysis necessary for these meta-games.

